Efficient Parallel Linear Scaling Method to get the Response Density Matrix in All-Electron Real-Space Density-Functional Perturbation Theory

The real-space density-functional perturbation theory (DFPT) for the computations of the response properties with respect to the atomic displacement and homogeneous electric field perturbation has been recently developed and implemented into the all-electron, numeric atom-centered orbitals electronic structure package FHI-aims. It is found that the bottleneck for large scale applications is the computation of the response density matrix, which scales as $O(N^3)$. Here for the response properties with respect to the homogeneous electric field, we present an efficient parallel linear scaling algorithm for the response density matrix calculation. Our scheme is based on the second-order trace-correcting purification and the parallel sparse matrix-matrix multiplication algorithms. The new scheme reduces the formal scaling from $O(N^3)$ to $O(N)$, and shows good parallel scalability over tens of thousands of cores. As demonstrated by extensive validation, we achieve a rapid computation of accurate polarizabilities using DFPT. Finally, the computational efficiency of this scheme has been illustrated by making the scaling tests and scalability tests on massively parallel computer systems.

==> Makefile <==
base_name := manuscript
datestamp := $(shell date +"%Y-%m-%d")
workdir   := $(shell basename $(shell pwd))


%.pdf: %.tex
	pdflatex --interaction=nonstopmode $<
	bibtex $*.aux
	pdflatex --interaction=nonstopmode $<
	pdflatex --interaction=nonstopmode $<


all: $(base_name).pdf  
	(evince $(base_name).pdf  &)


$(base_name).pdf: $(base_name).tex $(base_name).bib 

figures:
	$(MAKE) -C figures

dated:
	[ ! -d archive ] && mkdir archive
	$(MAKE) pdf
	cp -a $(base_name).pdf archive/$(base_name)-$(datestamp).pdf

tgz:
	$(MAKE) clean
	cd .. && tar -zcvf $(base_name)-$(datestamp).tgz $(workdir)

backup:
	$(MAKE) tgz
	cd .. && rsync -avizP $(base_name)-$(datestamp).tgz barin:backup/.

semiclean:
	rm -f *~ *.aux *.bbl *.blg *.brf *.bmt *.dvi *.log *.toc \
	$(base_name).pdf $(base_name).ps $(base_name).out $(base_name)Notes.bib

figuresclean:
	$(MAKE) -C figures clean

clean:
	$(MAKE) semiclean

.PHONY: clean figuresclean semiclean backup

